Summaries for Context-Free Games

We study two-player games played on the infinite graph of sentential forms induced by a context-free grammar (that comes with an ownership partitioning of the non-terminals). The winning condition is inclusion of the derived terminal word in the language of a finite automaton. Our contribution is a new algorithm to decide the winning player and to compute her strategy. It is based on a novel representation of all plays starting in a non-terminal. The representation uses the domain of Boolean formulas over the transition monoid of the target automaton. The elements of the monoid are essentially procedure summaries, and our approach can be seen as the first summary-based algorithm for the synthesis of recursive programs. We show that our algorithm has optimal (doubly exponential) time complexity, that it is compatible with recent antichain optimizations, and that it admits a lazy evaluation strategy. Our preliminary experiments indeed show encouraging results, indicating a speed up of three orders of magnitude over a competitor.

==> style/algo.tex <==
% ############
% ALGORITHMS
% ############

% algorithms
\usepackage{algorithmicx}
\usepackage{algpseudocode}

% code for "indentation guide"-style verticle lines
\makeatletter
\def\therule{\makebox[\algorithmicindent][l]{\hspace*{.5em}\vrule height .75\baselineskip depth .25\baselineskip}}%

\newtoks\therules% Contains rules
\therules={}% Start with empty token list
\def\appendto#1#2{\expandafter#1\expandafter{\the#1#2}}% Append to token list
\def\gobblefirst#1{% Remove (first) from token list
  #1\expandafter\expandafter\expandafter{\expandafter\@gobble\the#1}}%

\let\oldState\State
\def\LState{\oldState\unskip\the\therules}% New line-state
\let\State\LState
\let\Cmd\LState

\def\pushindent{\appendto\therules\therule}%
\def\popindent{\gobblefirst\therules}%
\def\printindent{\unskip\the\therules}%
\def\printandpush{\printindent\pushindent}%
\def\popandprint{\popindent\printindent}%

\algdef{SE}[WHILE]{While}{EndWhile}[1]
  {\printandpush\algorithmicwhile\ #1\ \algorithmicdo}
  {\popandprint\algorithmicend\ \algorithmicwhile}%
\algdef{SE}[FOR]{For}{EndFor}[1]
  {\printandpush\algorithmicfor\ #1\ \algorithmicdo}
  {\popandprint\algorithmicend\ \algorithmicfor}%
\algdef{S}[FOR]{ForAll}[1]
  {\printindent\algorithmicforall\ #1\ \algorithmicdo}%
\algdef{SE}[LOOP]{Loop}{EndLoop}
  {\printandpush\algorithmicloop}
  {\popandprint\algorithmicend\ \algorithmicloop}%
\algdef{SE}[REPEAT]{Repeat}{Until}
  {\printandpush\algorithmicrepeat}[1]
  {\popandprint\algorithmicuntil\ #1}%
\algdef{SE}[IF]{If}{EndIf}[1]
  {\printandpush\algorithmicif\ #1\ \algorithmicthen}
  {\popandprint\algorithmicend\ \algorithmicif}%
\algdef{C}[IF]{IF}{ElsIf}[1]
  {\popandprint\pushindent\algorithmicelse\ \algorithmicif\ #1\ \algorithmicthen}%
\algdef{Ce}[ELSE]{IF}{Else}{EndIf}
  {\popandprint\pushindent\algorithmicelse}%
\algdef{SE}[PROCEDURE]{Procedure}{EndProcedure}[2]
   {\printandpush\algorithmicprocedure\ \textproc{#1}\ifthenelse{\equal{#2}{}}{}{(#2)}}%
   {\popandprint\algorithmicend\ \algorithmicprocedure}%
\algdef{SE}[FUNCTION]{Function}{EndFunction}[2]
   {\printandpush\algorithmicfunction\ \textproc{#1}\ifthenelse{\equal{#2}{}}{}{(#2)}}%
   {\popandprint\algorithmicend\ \algorithmicfunction}%
\makeatother

% C-style comments
\renewcommand {\algorithmiccomment}[1]
    {\hfill $/ \!/$ #1}
   
% return on new line
\let\oldReturn\Return
\renewcommand{\Return}{\LState\oldReturn}

% commands like in algorith2e
\newcommand {\ForLoop} [2]
{
    \For {#1}
        #2
    \EndFor
}

\newcommand {\WhileLoop} [2]
{
    \While {#1}
        #2
    \EndWhile
}

\newcommand {\IfCond} [2]
{
    \If {#1}
        #2
    \EndIf
}

\newcommand {\IfElseCond} [3]
{
    \If {#1}
        #2
    \Else
        #3
    \EndIf
}

% environments
\newenvironment {forenv} [1]
{
    \For { #1 }
}
{ 
    \EndFor
}

    
\newenvironment {whileenv} [1]
{
    \While { #1 }
}
{ 
    \EndWhile
}

\newenvironment {ifenv} [1]
{
    \If { #1 }
}
{ 
    \EndIf
}


==> style/article.tex <==
% ########################
% ARTICLE SPECIFIC STUFF
% ########################

% Festlegung Art der Zitierung - Havardmethode: Abkuerzung Autor + Jahr
\usepackage[style=alphabetic,backend=bibtex]{biblatex}

% underlining
\usepackage{ulem}

% spacing between lines of text
\usepackage{setspace}

% enumerate etc
\usepackage{paralist}

% keyword index
\usepackage{makeidx}

% create keyword index
\makeindex

%% abbreviation index
%\usepackage[german]{nomencl}
%\let\abbrev\nomenclature

% border size
\usepackage{geometry}
\geometry{left=2.5cm, right=2.5cm, top=2cm, bottom=2cm, foot= 1cm}

% Indentation
% space between lines
\onehalfspacing
\renewcommand{\hmmax}{0}
\renewcommand{\bmmax}{0}
\clubpenalty = 10000 % Disable single lines at the start of a paragraph (Schusterjungen)
\widowpenalty = 10000 % Disable single lines at the end of a paragraph (Hurenkinder)
\displaywidowpenalty = 10000

% Schaltet den zusätzlichen Zwischenraum ab, den LaTeX normalerweise nach einem Satzzeichen einfügt.
%\frenchspacing

% references
\usepackage[bookmarksnumbered]{hyperref} 

% line break in URLs
%\usepackage[hyphens,obeyspaces,spaces]{url}

% newline after paragraph, paragraph bold and underlined
\makeatletter
\renewcommand {\paragraph}
{
    \@startsection
        {paragraph} % name
        {4}         % level
        {\z@}       % indent     
        {0ex \@plus -1ex \@minus -.2ex} % beforeskip
        %{-3.25ex\@plus -1ex \@minus -.2ex} % beforeskip
        {0.01ex \@plus .2ex}                % afterskip
        %{1.5ex \@plus -2ex}                % afterskip
        {\normalfont\normalsize\bfseries\underbar} % style of heading
}
\makeatother

% proof in bold font, colon and newline afterwards
\makeatletter
\renewenvironment{proof}[1][\proofname]
{
    \par
    \pushQED{\qed}%
    \normalfont \topsep6\p@\@plus6\p@\relax
    \trivlist
    \item[\hskip\labelsep\bfseries
    #1:]\mbox{}\\*\ignorespaces% ADDED
}
{
    \popQED\endtrivlist\@endpefalse
}
\makeatother

% set emph back to normal (instead of underlined)
\normalem 

% emph as bold
\makeatletter
\DeclareRobustCommand{\em}{%
    \@nomath\em \if b\expandafter\@car\f@series\@nil
    \normalfont \else \bfseries \fi}
\makeatother

% Theorem numbering
\def\theoremnumberstyle{changesection}

% Bei Nummerierung vom Typ swapped soll abweichend vom Standard
% "5.12. Satz" erscheinen als "5.12 Satz", das heisst ohne
% zusaetzlichen Punkt.
\makeatletter
\def\swappedhead#1#2#3{%
    \thmnumber{#2}\thmname{ #1}%
    \thmnote{ {\the\thm@notefont(#3)}}}
\makeatother

% Theoremstyle
\newtheoremstyle{varthm-roman-break} % name
{0.4cm}                          % Space above
{0.6cm}                          % Space below
{\normalfont}                    % Body font
{}                               % Indent amount
{\bfseries\sffamily}             % Theorem head font
{\newline}                       % Punctuation after theorem head
{0.2cm}                          % Space after theorem head
{\thmnote{#3}}                   % Theorem head spec


\swapnumbers
\theoremstyle{varthm-roman-break} 

% itemize/enumerate at the beginning of a thm
\newenvironment{thmenumerate}
{
    \leavevmode\vspace{-1.4em}
    \begin{enumerate}
    }
    {
    \end{enumerate}
}

\newenvironment{thmitemize}
{
    \leavevmode\vspace{-1.4em}
    \begin{itemize}
    }
    {
    \end{itemize}
}

% chapters = sections (otherwise numbering will not work)
\let\chapter\section

% subsections numbered by capital arabic letters
%\renewcommand{\thesubsection}{\thesection.\Roman{subsection}}
\renewcommand{\thesubsection}{\Alph{subsection})}

\usepackage{secdot}
\sectionpunct{subsection}{ }

% captions
\usepackage{capt-of}
\usepackage{caption}
\DeclareCaptionFont{white}{\color{white}}
\DeclareCaptionFormat{listing}
{
    \colorbox[cmyk]{1, 1, 1,0.01}
    {
        \parbox{\textwidth}
        {\hspace{15pt}#1#2#3}
    }
}
%\captionsetup[lstlisting]
%{
%    format=listing,
%    labelfont=white,
%    textfont=white,
%    singlelinecheck=false,
%    margin=0pt,
%    font={bf,footnotesize}
%}

% listings
\usepackage{listings}
\lstset{
    numbers=left,
    numberstyle=\tiny,
    numbersep=5pt,
    keywordstyle=\color{black}\bfseries,
    stringstyle=\ttfamily,
    showstringspaces=false,
    basicstyle=\footnotesize,
    captionpos=b
}
\lstset{language=java}
% Listings
\lstset{
    basicstyle=\fontsize{9}{9}\ttfamily, % Standardschrift
    numbers=left,               % Ort der Zeilennummern
    numberstyle=\tiny,          % Stil der Zeilennummern
    %stepnumber=2,               % Abstand zwischen den Zeilennummern
    numbersep=5pt,              % Abstand der Nummern zum Text
    tabsize=4,                  % Groesse von Tabs
    extendedchars=true,         %
    breaklines=true,            % Zeilen werden Umgebrochen
    keywordstyle=\text,
    %frame=b,         
    stringstyle=\color{black}\ttfamily, % Farbe der String
    showspaces=false,           % Leerzeichen anzeigen ?
    showtabs=false,             % Tabs anzeigen ?
    xleftmargin=5pt,
    framexleftmargin=17pt,
    framexrightmargin=5pt,
    framexbottommargin=4pt,
    %backgroundcolor=\color{lightgray},
    showstringspaces=false,      % Leerzeichen in Strings anzeigen ?
    captionpos=t,     
}

\lstloadlanguages{% Check Dokumentation for further languages ...
    %[Visual]Basic
    %Pascal
    %C
    %C++
    %XML
    %HTML
    Java
}

\definecolor{myblue}{HTML}{3399FF}
\definecolor{mybluefaded}{HTML}{99CCFF}
\definecolor{myred}{HTML}{FF3333}
\definecolor{myredfaded}{HTML}{FF9999}



==> style/commands.tex <==
% ##########
% COMMANDS
% ##########

% custom emph
\newcommand {\emphbf}[1]
{ \emph{#1} }

% bold + italic
\newcommand {\textbfit} [1]
{ \textbf{\textit{#1}} }

% monospace (+ bold & italic)
\newcommand {\mono} [1]
{ \texttt {#1} }

\newcommand {\monobf} [1]
{ \texttt {\bfseries #1} }

\newcommand {\monobfit} [1]
{ \texttt {\bfseries \itshape #1} }

\newcommand {\monoit} [1]
{ \texttt {\itshape #1} }

% fake capital greek letters
\newcommand {\Alpha} {A}
\newcommand {\Beta} {B}
\newcommand {\Epsilon} {E}
\newcommand {\Zeta} {Z}
\newcommand {\Eta} {H}
\newcommand {\Iota} {I}
\newcommand {\Kappa} {K}
\newcommand {\Mu} {M}
\newcommand {\Tau} {T}
\newcommand {\Chi} {X}

\providecommand\B{}
\renewcommand {\B} {{\mathbb B}}
\newcommand {\N} {{\mathbb N}}
\newcommand {\A} {{\mathbb A}}
\newcommand {\Z} {{\mathbb Z}}
\newcommand {\R} {{\mathbb R}}
\providecommand{\C}{}
\renewcommand {\C} {{\mathbb C}}
\newcommand {\Q} {{\mathbb Q}}
\newcommand {\D} {{\mathbb D}}
\newcommand {\F} {{\mathbb F}}
\newcommand {\E} {{\mathbb E}}
\providecommand {\G} {}
\renewcommand {\G} {{\mathbb G}}
\newcommand {\K} {{\mathbb K}}
\newcommand {\V} {{\mathbb V}}
\renewcommand {\P} {{\mathbb P}}
\renewcommand {\H} {{\mathbb H}}

% caligraphic letters
\newcommand {\calA} {\mathcal{A}}
\newcommand {\calB} {\mathcal{B}}
\newcommand {\calC} {\mathcal{C}}
\newcommand {\calD} {\mathcal{D}}
\newcommand {\calE} {\mathcal{E}}
\newcommand {\calF} {\mathcal{F}}
\newcommand {\calG} {\mathcal{G}}
\newcommand {\calH} {\mathcal{H}}
\newcommand {\calI} {\mathcal{I}}
\newcommand {\calJ} {\mathcal{J}}
\newcommand {\calK} {\mathcal{K}}
\newcommand {\calL} {\mathcal{L}}
\newcommand {\calM} {\mathcal{M}}
\newcommand {\calN} {\mathcal{N}}
\newcommand {\calO} {\mathcal{O}}
\newcommand {\calP} {\mathcal{P}}
\newcommand {\calQ} {\mathcal{Q}}
\newcommand {\calR} {\mathcal{R}}
\newcommand {\calS} {\mathcal{S}}
\newcommand {\calT} {\mathcal{T}}
\newcommand {\calU} {\mathcal{U}}
\newcommand {\calV} {\mathcal{V}}
\newcommand {\calW} {\mathcal{W}}
\newcommand {\calX} {\mathcal{X}}
\newcommand {\calY} {\mathcal{Y}}
\newcommand {\calZ} {\mathcal{Z}}


==> style/definitions.tex <==
% ##################
% DEFINITIONS
% ##################


%
% Stuff with dots
%

\newcommand{\wrt}
{wrt.\ }

\newcommand{\ie}
{i.e.\ }

\newcommand{\eg}
{e.g.\ }

\newcommand{\resp}
{resp.\ }

%
% Basic stuff
%

\newcommand { \from }
{ \leftarrow }

\newcommand {\Rplus} 
{ \R_{>0} }

\newcommand {\true}
{\mono{true}}

\newcommand {\false}
{\mono{false}}

\newcommand { \ifalse }
{ \mathit{false} }

\newcommand { \itrue }
{ \mathit{true} }

\newcommand {\oneto} [1]
{\left\{ 1, \ldots, #1\right\}}

\newcommand {\zeroto} [1]
{\left\{ 0, \ldots, #1\right\}}

\newcommand {\arity} [1]
{ {\scriptstyle / #1 } }

% matrix dimensions
\newcommand {\sz} [2]
{ #1 \raisebox{0.5pt} {\text{\;\!\tiny x\;\!}} #2}

\newcommand {\nsz} [2]
{ #1 \raisebox{0.5pt} {\text{\;\!\small x\;\!}} #2}

% small @
\newcommand {\at}
{
    \raisebox{0.5mm}{\scalebox{0.7}[0.7]{@}}
}

% corresponds to
\newcommand\corrto{%
    \let\savearraystretch\arraystretch
    \renewcommand\arraystretch{0.3}
    \begin{array}{c}
        \stretchto{
            \scalerel*[\widthof{=}]{\wedge}
            {\rule{1ex}{3ex}}%
        }{0.5ex}\\ 
        =%
    \end{array}
    \let\arraystretch\savearraystretch
}

% stacked logical operators
\newcommand{\wedgevee}
{
    \mathrel{\substack{\wedge\\\vee}}
}
\newcommand{\veewedge}
{
    \mathrel{\substack{\vee\\\wedge}}
}

\newcommand{\poly}
{\mathrm{poly}}

% small mid for (E)BNF
\newcommand{\bnf}
{\:\shortmid\:}

%
% Sets
%

\newcommand{\card}[1]
{\left|#1\right|}

\newcommand {\set} [1]
{ \left\{ #1 \right\} }

\newcommand {\Set} [2]
{ \left\{ #1 \ \middle| \ #2 \right\} }

\newcommand {\smallset} [2]
{ \{ #1 \mid #2 \} }

\newcommand {\ideal} [1]
{ \langle \ #1 \ \rangle}

\newcommand {\Ideal} [2]
{ \langle \ #1 \mid #2 \ \rangle}

\newcommand {\pwrset} [1]
{ {\mathcal P} \left( #1 \right)}

%
% Set operations
%

\newcommand* {\medcap}
{ \mathbin{\scalebox{1.5}{\ensuremath{\cup}}} }
\newcommand* {\medcup}
{ \mathop{\mathbin{\scalebox{1.5}{\ensuremath{\cup}}}} } 
\newcommand* {\hugecup}
{ \mathop{\mathbin{\scalebox{3}{\ensuremath{\cup}}}} }

\newcommand {\bigdotcup}
{\ensuremath{\mathop{\mathaccent\cdot{\bigcup}}}}
\newcommand {\dotcup}
{\ensuremath{\mathop{\mathaccent\cdot\cup}}}

% disjoint union
\makeatletter
\providecommand*{\bigcupdot}{%
    \mathbin{%
        \mathpalette\@bigcupdot{}%
    }%
}
\newcommand*{\@bigcupdot}[2]{%
    \ooalign{%
        $\m@th#1\bigcup$\cr
        \hidewidth$\m@th#1\cdot$\hidewidth
    }%
}
\makeatother

\makeatletter
\providecommand*{\cupdot}{%
    \mathbin{%
        \mathpalette\@cupdot{}%
    }%
}
\newcommand*{\@cupdot}[2]{%
    \ooalign{%
        $\m@th#1\cup$\cr
        \hidewidth$\m@th#1\cdot$\hidewidth
    }%
}
\makeatother

\newcommand{\up}
{\!\uparrow}

\newcommand{\down}
{\!\downarrow}

\newcommand{\dc}[1]
{#1\!\downarrow\ }

\newcommand{\uc}[1]
{#1\!\uparrow\ }

%
% Logic
%
\newcommand {\Fzero} {\calF_0}
\newcommand {\dedFzero} {\vdash_{\calF_0}}
\DeclareDocumentCommand \FO { g } % optinal argument in curly braces
{ 
    \IfNoValueTF {#1}
    { \text{FO} }
    { \text{FO} \left( #1 \right) }
}
\newcommand {\dedG} {\vdash_{G}}
\newcommand {\dedRes} {\vdash_{\mathit{Res}}}
\newcommand {\sem}[1]
{	\left\llbracket #1 \right\rrbracket }
\newcommand {\Sko} {\mathsf{Sko}}
\DeclareDocumentCommand \FOneq { g } % optinal argument in curly braces
{ 
    \IfNoValueTF {#1}
    { \text{FO}^{\neq} }
    { \text{FO}^{\neq} \left( #1 \right) }
}
\DeclareDocumentCommand \FOcl { g } % optinal argument in curly braces
{ 
    \IfNoValueTF {#1}
    { \text{FO}_{\mathit{abg}} }
    { \text{FO}_{\mathit{abg}} \left( #1 \right) }
}
\newcommand {\Dherbrand} {D_{\calH}}

% inverse models
\makeatletter
\providecommand*{\Dashv}{%
    \mathrel{%
        \mathpalette\@Dashv\vDash
    }%
}
\newcommand*{\@Dashv}[2]{%
    \reflectbox{$\m@th#1#2$}%
}
\makeatother

% logical equivalence (\models \ismod)
\newcommand{\lequiv}{\vDash\hspace{-2pt}\Dashv}

% cons / folg
\DeclareMathOperator {\Folg} {Folg}
\DeclareMathOperator {\Cons} {Cons}


%
% Complexity
%

\newcommand {\bigO} [1]
{ \calO \left( {#1} \right) }

\newcommand {\smallO} [1]
{ o \left( #1 \right) }

\newcommand {\bigOmega} [1]
{ \Omega \left( #1 \right) }

\newcommand {\smallOmega} [1]
{ \omega \left( #1 \right) }

\newcommand {\bigTheta} [1]
{ \Theta \left( #1 \right) }

% blank symbol
%\newsavebox{\textvisiblespacebox}
%\savebox{\textvisiblespacebox}{\texttt{a}}
%\newcommand\vartextvisiblespace[1][\wd\textvisiblespacebox]{%
%    \makebox[#1]{\kern.1em\rule{.4pt}{.3ex}%
%        \hrulefill%
%        \rule{.4pt}{.3ex}\kern.1em}%
%}
%\newcommand{\blank}{\vartextvisiblespace}% For ease-of-use
\newcommand{\blank}{\texttt{\char32}}% For ease-of-use

\newcommand {\LOGSPACE}
{$\mathsf{L}$}
\newcommand {\NLOGSPACE}
{$\mathsf{NL}$}
\newcommand {\PTIME}
{$\mathsf{P}$}
\newcommand {\NPTIME}
{$\mathsf{NP}$}
\newcommand {\PSPACE}
{$\mathsf{PSPACE}$}
\newcommand {\EXPTIME}
{$\mathsf{EXP}$}
\newcommand {\EXPSPACE}
{$\mathsf{EXPSPACE}$}

%
% Graphs
%

\newcommand {\paths} [2]
{ { \calP \left( {#1}, {#2} \right)} }

\newcommand {\cycles} [1]
{ \calC \left( #1 \right)}

\newcommand {\cyclesne} [1]
{ \calC^{\neq \epsilon} \left( #1 \right)}

%
% Words
%

\newcommand{\prefix}[1]
{\text{prefix}(#1)}

\newcommand {\subword}
{\!\preceq}

%
% Automata theory
%

\newcommand {\tow} [1]
{ \overset{#1}{\to} }

\newcommand{\towi}[2]
{\tow{#1}_{#2}}

\DeclareDocumentCommand \lang { g } % optinal argument in curly braces
{ 
    \IfNoValueTF {#1}
    { \calL }
    { \calL \left( #1 \right) }
}
\newcommand {\langm}
{ \calM }
\DeclareDocumentCommand \olang { g } % optinal argument in curly braces
{ 
    \IfNoValueTF {#1}
    { \calL^\omega }
    { \calL^\omega \!\left( #1 \right) }
}

\DeclareDocumentCommand \Parikh { g } % optinal argument in curly braces
{ 
    \IfNoValueTF {#1}
    { \Psi }
    { \Psi \left( #1 \right) }
}

\DeclareMathOperator {\Boxes} {M}

\newcommand{\WMSO}{WMSO}
\DeclareMathOperator{\suc}{suc}
\newcommand{\WDSO}{WDSO}
\newcommand{\WMSONull}{\WMSO_0}

\newcommand {\Prio}[1]{\Omega \left(#1\right)}

%
% Petri nets
%

\newcommand {\TEnable}[3]
{{#1\lbrack #2 \rangle #3}}

\newcommand {\TJustEnable}[2]
{{#1\lbrack #2 \rangle}}

% 
% Algebraic geometry, Computer algebra
% 

\providecommand{\x}{}
\renewcommand {\x} {\underline{x}}
\newcommand {\xs} {\underline{xs}}
\newcommand {\p} {\underline{p}}

\newcommand {\polyr} { K [ \x ] }

\newcommand {\polyrQ} { \Q [ \x ] }
\newcommand {\polyrC} { \C [ \x ] }

\newcommand {\polyrs} { K [ \xs ] }
\newcommand {\polyrwo} [1]
{ K [ x_j \ | \ j \neq #1 \ ] }
\newcommand {\polyrwoi} { K [ x_j \ | \ j \neq i \ ] }
\newcommand {\polyrQwoi} { \Q [ x_j \ | \ j \neq i \ ] }
\newcommand {\polyrQwo} [1]
{ \Q [ x_j \ | \ j \neq #1 \ ] }

\newcommand {\laurentr} { K [ \x^{\pm 1} ] }
\newcommand {\laurentrQ} { \Q [ \x^{\pm 1} ] }

\newcommand {\Qxs} { \Q [ \xs ] }

\newcommand {\tropring} {(\R \cup \{ -\infty\})}

\newcommand {\aff} [2] {\A ^{#1} _{#2}}
\newcommand {\affn} [1] {\A ^{n} _{#1}}
\newcommand {\affnk} {\A ^{n} _{K}}

\newcommand {\projs} [2] {\P ^{#1} _{#2}}
\newcommand {\projn} [1] {\P ^{n} _{#1}}
\newcommand {\projnK} {\P ^{n} _{K}}

\newcommand {\tor} [2]
{T ^{#1} _{#2}}
\newcommand {\torn} [1]
{T ^{n} _{#1}}
\newcommand {\tornK} {T ^{n} _{K}}

\newcommand {\puis} [1]
{#1\{ \! \{t\} \! \}}
\newcommand {\puisK} {K\{ \! \{t\} \! \}}
\newcommand {\puisC} {\C\{  \! \{t\} \! \}}

\DeclareMathOperator {\LT} {LT}
\DeclareMathOperator {\LC} {LC}
\DeclareMathOperator {\LM} {LM}

\DeclareMathOperator {\InitOp} {in}
\newcommand {\Init} [2]
{ \InitOp_{#1} \left( #2 \right)}

\DeclareMathOperator {\troppoly} {troppoly}

\DeclareMathOperator {\TropOp} {Trop}
\newcommand {\Trop} [1]
{ \TropOp \left( #1 \right)}

%
% Polyhedrons
%

\DeclareMathOperator {\cone} {cone}

\DeclareMathOperator {\IntOp} {Int}
\newcommand {\Int} [1]
{ \IntOp \left( #1 \right)}

\DeclareMathOperator {\RelIntOp} {relInt}
\newcommand {\RelInt} [1]
{ \RelIntOp \left( #1 \right)}

\DeclareMathOperator {\Suppop} {Supp}
\newcommand {\Supp} [1]
{\Suppop \left( #1 \right)}

%
% Master thesis specific
%

\newcommand {\subsets} [2]
{ \Lambda\left(#1, #2\right) }

\DeclareMathOperator {\BoundeOp} {Bound^e}
\newcommand {\Bounde} [2]
{ \BoundeOp_{#1} \left( #2 \right) }
\newcommand {\Boundei} [1]
{ \Bounde{i} {#1}}
\newcommand {\Boundes} [1]
{ \Bounde{1} {#1}}

\DeclareMathOperator {\BoundpOp} {Bound^p}
\newcommand {\Boundp} [2]
{ \BoundpOp_{#1} \left( #2 \right) }
\newcommand {\Boundpi} [1]
{ \Boundp{i} {#1}}
\newcommand {\Boundps} [1]
{ \Boundp{1} {#1}}

%
% Special formatting
%

\newcommand {\singular} {S\textsc{ingular} }
\newcommand {\Buechi} {{B\"uchi }}

%
% Antichains for Inclusion Games
%

% derivation
\newcommand{\derive}{\Rightarrow}
\newcommand{\leftderive}{\derive_L}

% transition boxes
\newcommand {\tboxr}
{ \rho }
\newcommand {\tboxt}
{ \tau }
\newcommand {\tbox} [1]
{ \rho_{#1} }
\newcommand {\var} [1]
{ \Delta_{#1} }
\newcommand {\sol} [1]
{ \sigma_{#1} }

% "fake" identity
\newcommand {\fid}
{ \id }

% CNF formulas
\DeclareMathOperator {\CNF}
{ CNF }
\newcommand {\CNFE}
{ \CNF \! /_{\lsim}}

% positive formulas over boxes
\DeclareMathOperator {\BF}
{ BF }
\newcommand {\BFE}
{ \BF \! /\!_{\lsim}}

% singleton formula
\newcommand {\snglt} [1]
{ \set{ \set{ #1 } } }

% special orders
\newcommand {\lleq}
{ \Rightarrow}
%{ \models}
\newcommand {\lsim}
{ \Leftrightarrow }
%{ \lequiv }

\newcommand {\natlt}
{ \prec }
\newcommand {\natgt}
{ \succ }

\newcommand{\stateequiv} [1]
{\sim_{#1}}

% winning regions and strategies
\newcommand {\wrinclusion}
{W^{\subseteq \calL (A) }}
\newcommand {\wrnoninclusion}
{W^{\not\subseteq \calL (A) }}

\newcommand {\wstratemptiness}
{s^{= \emptyset}}
\newcommand {\wstratnonemptiness}
{s^{\neq \emptyset}}
\newcommand {\wstratinclusion}
{s^{\subseteq \lang{A} }}
\newcommand {\wstratnoninclusion}
{s^{\not\subseteq \lang{A} }}

% players
\newcommand {\round} { {\raisebox{0.1em}{{\mbox{\scaleobj{0.8}{\bigcirc}}}}} }
\newcommand {\roundss} { {\raisebox{0.1em}{{\mbox{\scaleobj{0.65}{\bigcirc}}}}} }

\newcommand {\players} { \set{\round, \square}}

\newcommand\openbigstar[1][0.7]{
    {
        \scalerel*{%
            \stackinset{c}{-.125pt}{c}{}{\scalebox{#1}{\color{white}{$\bigstar$}}}{%
                $\bigstar$}%
        }{\bigstar}
    }
}
\newcommand {\player} { {\openbigstar} }
\newcommand {\opponent} { \overline{\openbigstar} }

% other stuff
\newcommand {\ChosenBoxes} { \Set{ c(K) }{ K \in F }  }

\newcommand {\lvl}
{\mathit{lvl}} 

\DeclareDocumentCommand \level { g } % optoinal argument in curly braces
{ 
    \IfNoValueTF {#1}
    { \mathit{level } }
    { \mathit{level} \left( #1 \right) }
}

\DeclareDocumentCommand \FT { g g } % two optional arguments in curly braces
{ 
    \IfNoValueTF {#1}
    {
        {\calT}
    }
    {
        \IfNoValueTF {#2}
        {
            {\calT_{#1}}
        }
        {
            {\calT_{#1}^{#2}}   
        }
    }
}

 %
 % Valence games
 %
 
 \newcommand{\inc}[1]
 {{#1}^+}
 
 \newcommand{\dec}[1]
 {{#1}^-}
 
 \newcommand{\ops}[1]
 {\inc{#1},\dec{#1}}
 
 \newcommand{\opset}
 {\calO}
 
 \newcommand{\oplang}
 {\opset^*}
 
 \newcommand{\opmonoid}
 {M_\opset}
 

==> style/exam.tex <==
% ########################
% EXAM SPECIFIC STUFF
% ########################

% Festlegung Art der Zitierung - Havardmethode: Abkuerzung Autor + Jahr
\usepackage[style=alphabetic,backend=bibtex]{biblatex}

% underlining
\usepackage{ulem}

% spacing between lines of text
\usepackage{setspace}

% enumerate etc
\usepackage{paralist}

% keyword index
\usepackage{makeidx}

% create keyword index
\makeindex

%% abbreviation index
%\usepackage[german]{nomencl}
%\let\abbrev\nomenclature

% border size
\usepackage{geometry}
\geometry{left=2.5cm, right=2.5cm, top=2cm, bottom=2cm, foot= 1cm}

% Indentation
% space between lines
\onehalfspacing
\renewcommand{\hmmax}{0}
\renewcommand{\bmmax}{0}
\clubpenalty = 10000 % Disable single lines at the start of a paragraph (Schusterjungen)
\widowpenalty = 10000 % Disable single lines at the end of a paragraph (Hurenkinder)
\displaywidowpenalty = 10000

% Schaltet den zusätzlichen Zwischenraum ab, den LaTeX normalerweise nach einem Satzzeichen einfügt.
%\frenchspacing

% references
\usepackage[bookmarksnumbered]{hyperref} 

% line break in URLs
%\usepackage[hyphens,obeyspaces,spaces]{url}

% newline after paragraph, paragraph bold and underlined
\makeatletter
\renewcommand {\paragraph}
{
    \@startsection
        {paragraph} % name
        {4}         % level
        {\z@}       % indent     
        {0ex \@plus -1ex \@minus -.2ex} % beforeskip
        %{-3.25ex\@plus -1ex \@minus -.2ex} % beforeskip
        {0.01ex \@plus .2ex}                % afterskip
        %{1.5ex \@plus -2ex}                % afterskip
        {\normalfont\normalsize\bfseries\underbar} % style of heading
}
\makeatother

% proof in bold font, colon and newline afterwards
\makeatletter
\renewenvironment{proof}[1][\proofname]
{
    \par
    \pushQED{\qed}%
    \normalfont \topsep6\p@\@plus6\p@\relax
    \trivlist
    \item[\hskip\labelsep\bfseries
    #1:]\mbox{}\\*\ignorespaces% ADDED
}
{
    \popQED\endtrivlist\@endpefalse
}
\makeatother

% set emph back to normal (instead of underlined)
\normalem 

% emph as bold
\makeatletter
\DeclareRobustCommand{\em}{%
    \@nomath\em \if b\expandafter\@car\f@series\@nil
    \normalfont \else \bfseries \fi}
\makeatother

% Theorem numbering
\def\theoremnumberstyle{changesection}

% Bei Nummerierung vom Typ swapped soll abweichend vom Standard
% "5.12. Satz" erscheinen als "5.12 Satz", das heisst ohne
% zusaetzlichen Punkt.
\makeatletter
\def\swappedhead#1#2#3{%
    \thmnumber{#2}\thmname{ #1}%
    \thmnote{ {\the\thm@notefont(#3)}}}
\makeatother

% Theoremstyle
\newtheoremstyle{varthm-roman-break} % name
{0.4cm}                          % Space above
{0.6cm}                          % Space below
{\normalfont}                    % Body font
{}                               % Indent amount
{\bfseries\sffamily}             % Theorem head font
{\newline}                       % Punctuation after theorem head
{0.2cm}                          % Space after theorem head
{\thmnote{#3}}                   % Theorem head spec


\swapnumbers
\theoremstyle{varthm-roman-break} 

% itemize/enumerate at the beginning of a thm
\newenvironment{thmenumerate}
{
    \leavevmode\vspace{-1.4em}
    \begin{enumerate}
    }
    {
    \end{enumerate}
}

\newenvironment{thmitemize}
{
    \leavevmode\vspace{-1.4em}
    \begin{itemize}
    }
    {
    \end{itemize}
}

% chapters = sections (otherwise numbering will not work)
\let\chapter\section

% subsections numbered by capital arabic letters
%\renewcommand{\thesubsection}{\thesection.\Roman{subsection}}
\renewcommand{\thesubsection}{\Alph{subsection})}

\usepackage{secdot}
\sectionpunct{subsection}{ }

% captions
\usepackage{capt-of}
\usepackage{caption}
\DeclareCaptionFont{white}{\color{white}}
\DeclareCaptionFormat{listing}
{
    \colorbox[cmyk]{1, 1, 1,0.01}
    {
        \parbox{\textwidth}
        {\hspace{15pt}#1#2#3}
    }
}
%\captionsetup[lstlisting]
%{
%    format=listing,
%    labelfont=white,
%    textfont=white,
%    singlelinecheck=false,
%    margin=0pt,
%    font={bf,footnotesize}
%}

% listings
\usepackage{listings}
\lstset{
    numbers=left,
    numberstyle=\tiny,
    numbersep=5pt,
    keywordstyle=\color{black}\bfseries,
    stringstyle=\ttfamily,
    showstringspaces=false,
    basicstyle=\footnotesize,
    captionpos=b
}
\lstset{language=java}
% Listings
\lstset{
    basicstyle=\fontsize{9}{9}\ttfamily, % Standardschrift
    numbers=left,               % Ort der Zeilennummern
    numberstyle=\tiny,          % Stil der Zeilennummern
    %stepnumber=2,               % Abstand zwischen den Zeilennummern
    numbersep=5pt,              % Abstand der Nummern zum Text
    tabsize=4,                  % Groesse von Tabs
    extendedchars=true,         %
    breaklines=true,            % Zeilen werden Umgebrochen
    keywordstyle=\text,
    %frame=b,         
    stringstyle=\color{black}\ttfamily, % Farbe der String
    showspaces=false,           % Leerzeichen anzeigen ?
    showtabs=false,             % Tabs anzeigen ?
    xleftmargin=5pt,
    framexleftmargin=17pt,
    framexrightmargin=5pt,
    framexbottommargin=4pt,
    %backgroundcolor=\color{lightgray},
    showstringspaces=false,      % Leerzeichen in Strings anzeigen ?
    captionpos=t,     
}

\lstloadlanguages{% Check Dokumentation for further languages ...
    %[Visual]Basic
    %Pascal
    %C
    %C++
    %XML
    %HTML
    Java
}

\definecolor{myblue}{HTML}{3399FF}
\definecolor{mybluefaded}{HTML}{99CCFF}
\definecolor{myred}{HTML}{FF3333}
\definecolor{myredfaded}{HTML}{FF9999}

\newcommand{\maxpts}[1]
{
    \vspace*{-1.5cm}
    \hfill \fbox{\large #1 \pts}
    \vspace*{1cm}
}

\RequirePackage{scrpage2}
\pagestyle{scrheadings}
\clearscrheadings
\ohead{\hfill \quad \normalfont \page{} \pagemark/\pageref{LastPage}}


% multiplechoice
\newenvironment{multiplechoice}[2]{
    \begin{center}
        \begin{tabular}{lcc}
            & #1 & #2 \\
        }{
    \end{tabular}
\end{center}
\vspace{0.5cm}
}


\newcommand{\statement}[1]{
    #1	& $\Box$ & $\Box$ \\
}

% for proofs
\usepackage{bussproofs}

\newenvironment{exerciseDE}[2]
{
    \newpage
    \section{#1}
    \maxpts{#2}
    \vspace*{-0.7cm}
    
}
{
}

\newenvironment{exerciseEN}[2]
{
    \newpage
    \section{#1}
    \maxpts{#2}
    \vspace*{-0.7cm}
        
}
{
}

\newenvironment{firstpage}
{
    \thispagestyle{empty}
    \newgeometry{top=1cm, bottom=1cm}
}
{
    \pagebreak
    \restoregeometry
}



==> style/exsheet.tex <==
% ##############################
% EXERCISE SHEET SPECIFIC STUFF
% ##############################

% Festlegung Art der Zitierung - Havardmethode: Abkuerzung Autor + Jahr
\usepackage[style=alphabetic,backend=bibtex]{biblatex}

% underlining
\usepackage{ulem}

% remove all paragraph indentation
\usepackage{parskip}

% spacing between lines of text
\usepackage{setspace}

% enumerate etc
\usepackage{paralist}

% keyword index
\usepackage{makeidx}

% create keyword index
\makeindex

% abbreviation index
\usepackage[german]{nomencl}
\let\abbrev\nomenclature

% border size
\usepackage{geometry}
\geometry{left=2.2cm, right=2.2cm, top=2cm, bottom=2cm, foot= 1cm}

% Indentation
% space between lines
\onehalfspacing
\renewcommand{\hmmax}{0}
\renewcommand{\bmmax}{0}
\clubpenalty = 10000 % Disable single lines at the start of a paragraph (Schusterjungen)
\widowpenalty = 10000 % Disable single lines at the end of a paragraph (Hurenkinder)
\displaywidowpenalty = 10000
% Schaltet den zusätzlichen Zwischenraum ab, den LaTeX normalerweise nach einem Satzzeichen einfügt.
\frenchspacing

%\usepackage{scrpage2}
%\pagestyle{scrheadings}
%\cfoot{\pagemark}

%  headline / footline
\usepackage{fancyhdr} %Paket laden
\pagestyle{fancy} %eigener Seitenstil

%% Seitennummer immer oben rechts
%% alle Kopf- und Fußzeilenfelder bereinigen
%\fancyhf{}
%% Kopfzeile links: Name des Kapitels = der Sektion
%\fancyhead[L]{\nouppercase{\leftmark}}
%% Kopfzeile zentriert:
%\fancyhead[C]{} 
%% Kopfzeile rechts = Seitennummer
%\fancyhead[R]{\thepage} 
%% Trennlinien
%\renewcommand{\headrulewidth}{0.4pt} 
%%\renewcommand{\footrulewidth}{0.4pt}
%% Analog
%%\fancyfoot[C]{\thepage}


% Seitennummer immer oben rechts
% alle Kopf- und Fußzeilenfelder bereinigen
\fancyhf{}
\fancyfoot[C]{}
\renewcommand{\headrule}{} 

% references
\usepackage[bookmarksnumbered]{hyperref} 

% line break in URLs
%\usepackage[hyphens,obeyspaces,spaces]{url}

% newline after paragraph, paragraph bold and underlined
\makeatletter
\renewcommand {\paragraph}
{
    \@startsection
        {paragraph} % name
        {4}         % level
        {\z@}       % indent     
        {0ex \@plus -1ex \@minus -.2ex} % beforeskip
        %{-3.25ex\@plus -1ex \@minus -.2ex} % beforeskip
        {0.01ex \@plus .2ex}                % afterskip
        %{1.5ex \@plus -2ex}                % afterskip
        {\normalfont\normalsize\bfseries\underbar} % style of heading
}
\makeatother

% proof in bold font, colon and newline afterwards
\makeatletter
\renewenvironment{proof}[1][\proofname]
{
    \par
    \pushQED{\qed}%
    \normalfont \topsep6\p@\@plus6\p@\relax
    \trivlist
    \item[\hskip\labelsep\bfseries
    #1:]\mbox{}\\*\ignorespaces% ADDED
}
{
    \popQED\endtrivlist\@endpefalse
}
\makeatother

% set emph back to normal (instead of underlined)
\normalem 

% emph as bold
\makeatletter
\DeclareRobustCommand{\em}{%
    \@nomath\em \if b\expandafter\@car\f@series\@nil
    \normalfont \else \bfseries \fi}
\makeatother

% Theorem numbering
%\def\theoremnumberstyle{changesection}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Zu verwendende Regelsaetze 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Bei Nummerierung vom Typ swapped soll abweichend vom Standard
%%% "5.12. Satz" erscheinen als "5.12 Satz", das heisst ohne
%%% zusaetzlichen Punkt.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\def\swappedhead#1#2#3{%
%    \thmnumber{#2}\thmname{\@ifnotempty{#2}{ }#1}%
%    \thmnote{ {\the\thm@notefont(#3)}}}

%\def\swappedhead#1#2#3{%
%    \thmnumber{#2}\thmname{ #1}%
%    \thmnote{ {\the\thm@notefont(#3)}}}


% Theoremstyle
\newtheoremstyle{varthm-roman-break} % name
{0.4cm}                    % Space above
{0.6cm}                    % Space below
{\normalfont}                   % Body font
{}                           % Indent amount
{\bfseries}                   % Theorem head font
{\newline}                          % Punctuation after theorem head
{0.2cm}                       % Space after theorem head
{#1 #2\thmnote{: \ #3}}  % Theorem head spec (can be left empty, meaning ‘normal’)


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Eigene Befehle
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Label an beliebiger Stelle mit beliebigem Symbol setzen
% \mylabel{labelname}{(*)} liefert (*) nach \ref{labelname}
\catcode`@=11%%% Sorgt daruer, dass @ in Marconamen verwendet werden kann
\newcommand{\mylabel}[2]{\@bsphack
    \protected@write\@auxout{}%
    {\string\newlabel{#1}{{#2}{\thepage}}}%
    \@esphack}
\newcommand{\tmylabel}[2]{\@bsphack
    \protected@write\@auxout{}%
    {\string\newlabel{#1}{{#2}{\thepage}{\arabic{chapter}}}}%
    \@esphack}
\catcode`@=\active%
%%% Erzeugt an der Stelle des Aufrufs einen nicht sichtbaren Punkt.
\newcommand{\leererpunkt}{
    \drawdim pt
    \begin{texdraw}
        \setgray 1
        \lcir r:0.01       
    \end{texdraw}
}

%\swapnumbers
\theoremstyle{varthm-roman-break} 

% itemize/enumerate at the beginning of a thm
\newenvironment{thmenumerate}
{
    \leavevmode\vspace{-1.4em}
    \begin{enumerate}
    }
    {
    \end{enumerate}
}

\newenvironment{thmitemize}
{
    \leavevmode\vspace{-1.4em}
    \begin{itemize}
    }
    {
    \end{itemize}
}

% chapters = sections (otherwise numbering will not work)
%\let\chapter\section

% subsections numbered by capital arabic letters
%\renewcommand{\thesubsection}{\thesection.\Roman{subsection}}
\renewcommand{\thesubsection}{\Alph{subsection})}

\usepackage{secdot}
\sectionpunct{subsection}{ }


% captions
\usepackage{capt-of}
\usepackage{caption}
\DeclareCaptionFont{white}{\color{white}}
\DeclareCaptionFormat{listing}
{
    \colorbox[cmyk]{1, 1, 1,0.01}
    {
        \parbox{\textwidth}
        {\hspace{15pt}#1#2#3}
    }
}
\captionsetup[lstlisting]
{
    format=listing,
    labelfont=white,
    textfont=white,
    singlelinecheck=false,
    margin=0pt,
    font={bf,footnotesize}
}

% listings
\usepackage{listings}
\lstset{
    numbers=left,
    numberstyle=\tiny,
    numbersep=5pt,
    keywordstyle=\color{black}\bfseries,
    stringstyle=\ttfamily,
    showstringspaces=false,
    basicstyle=\footnotesize,
    captionpos=b
}
\lstset{language=java}
% Listings
\lstset{
    basicstyle=\fontsize{9}{9}\ttfamily, % Standardschrift
    numbers=left,               % Ort der Zeilennummern
    numberstyle=\tiny,          % Stil der Zeilennummern
    %stepnumber=2,               % Abstand zwischen den Zeilennummern
    numbersep=5pt,              % Abstand der Nummern zum Text
    tabsize=4,                  % Groesse von Tabs
    extendedchars=true,         %
    breaklines=true,            % Zeilen werden Umgebrochen
    keywordstyle=\text,
    %frame=b,         
    stringstyle=\color{black}\ttfamily, % Farbe der String
    showspaces=false,           % Leerzeichen anzeigen ?
    showtabs=false,             % Tabs anzeigen ?
    xleftmargin=5pt,
    framexleftmargin=17pt,
    framexrightmargin=5pt,
    framexbottommargin=4pt,
    %backgroundcolor=\color{lightgray},
    showstringspaces=false,      % Leerzeichen in Strings anzeigen ?
    captionpos=t,     
}

\lstloadlanguages{% Check Dokumentation for further languages ...
    %[Visual]Basic
    %Pascal
    %C
    %C++
    %XML
    %HTML
    Java
}

\definecolor{myblue}{HTML}{3399FF}
\definecolor{mybluefaded}{HTML}{99CCFF}
\definecolor{myred}{HTML}{FF3333}
\definecolor{myredfaded}{HTML}{FF9999}

\newtoks\lecturer
\newtoks\organizer
\newtoks\institution
\newtoks\term
\newtoks\releasedate
\newtoks\duedate

\makeatletter
\newcommand{\head}
{
%   \newgeometry{top=1cm}
    \vspace*{-3\baselineskip}
    %\null
    %\thispagestyle{empty}
    %\begin{center} 
    \framebox{
        \parbox{\textwidth}
        {
            \vspace*{0.2cm}
            \begin{center}
                \textrm{\textbf{\large \@title}} \\
                \textrm{\textbf{\large \@subtitle}}
            \end{center}
            \vspace*{-0.5cm}
            \begin{tabu} to \textwidth {l X r}
                \small \the\lecturer  & & \small \the\institution \\
                \small \the\organizer  & & \small \the\term \\
            \end{tabu}
        }
    } 
    %\end{center}
    %\null
    \begin{tabu} to 1.025\columnwidth {@{} l X r @{}}
        \the\releasedate  & & \the \duedate \\
    \end{tabu}
%    \vspace*{0.2cm}
%    \restoregeometry
}
\makeatother



==> style/helvetica.tex <==
% #######
% HELVETICA
% #######

% Helvetica pro for text (and math)
% Consolas for monospace
% Euler for math

\usepackage{helvet}
\renewcommand{\familydefault}{\sfdefault}

\usepackage{isomath}
\usepackage{sansmathfonts}

% package to change font in XeTeX
%\usepackage[no-math]{fontspec}

% euler font for math
%\usepackage[mathbf]{euler}
    
% default font: Myriad pro
% (has to be installed!)
%\setmainfont{Myriad Pro}
%\newfontfamily\myriad{Myriad Pro}

% monospace font: Consolas
% (has to be installed!)
%\setmonofont{Consolas}

% use normal text font for math
%\usepackage[noendash]{mathastext}

% hack for emptyset
%\renewcommand{\emptyset}{ {\diameter} }

% font for section, part, ... titles (in text and in table of contents)
%\usepackage{titlesec}
%\setkomafont{subsection}{\bfseries\Large\myriad}
%\setkomafont{section}{\bfseries\huge\myriad}
%\setkomafont{sectionentry}{\bfseries\myriad} % entry in TOC
%\setkomafont{part}{\bfseries\Huge\myriad} % part name
%\setkomafont{partnumber}{\bfseries\Huge\myriad} % "Part II."
%\setkomafont{partentry}{\bfseries\large\myriad} % entry in TOC
%\setkomafont{paragraph}{\bfseries\myriad}
%\setkomafont{subparagraph}{\bfseries\myriad} % entry in TOC

% Take nice sans-serif greek letters from the font "Euler"
%\DeclareSymbolFont{EulerGreek}{U}{eur}{m}{n}
%\DeclareMathSymbol\Gamma    {\mathalpha}{EulerGreek}{"00}
%\DeclareMathSymbol\Delta    {\mathalpha}{EulerGreek}{"01}
%\DeclareMathSymbol\Theta    {\mathalpha}{EulerGreek}{"02}
%\DeclareMathSymbol\Lambda   {\mathalpha}{EulerGreek}{"03}
%\DeclareMathSymbol\Xi       {\mathalpha}{EulerGreek}{"04}
%\DeclareMathSymbol\Pi       {\mathalpha}{EulerGreek}{"05}
%\DeclareMathSymbol\Sigma    {\mathalpha}{EulerGreek}{"06}
%\DeclareMathSymbol\Upsilon  {\mathalpha}{EulerGreek}{"07}
%\DeclareMathSymbol\Phi      {\mathalpha}{EulerGreek}{"08}
%\DeclareMathSymbol\Psi      {\mathalpha}{EulerGreek}{"09}
%\DeclareMathSymbol\Omega    {\mathalpha}{EulerGreek}{"0A}
%\DeclareMathSymbol{\alpha}  {\mathalpha}{EulerGreek}{"0B}
%\DeclareMathSymbol{\beta}   {\mathalpha}{EulerGreek}{"0C}
%\DeclareMathSymbol{\gamma}  {\mathalpha}{EulerGreek}{"0D}
%\DeclareMathSymbol{\delta}  {\mathalpha}{EulerGreek}{"0E}
%\DeclareMathSymbol{\epsilon}{\mathalpha}{EulerGreek}{"0F}
%\DeclareMathSymbol{\zeta}   {\mathalpha}{EulerGreek}{"10}
%\DeclareMathSymbol{\eta}    {\mathalpha}{EulerGreek}{"11}
%\DeclareMathSymbol{\theta}  {\mathalpha}{EulerGreek}{"12}
%\DeclareMathSymbol{\iota}   {\mathalpha}{EulerGreek}{"13}
%\DeclareMathSymbol{\kappa}  {\mathalpha}{EulerGreek}{"14}
%\DeclareMathSymbol{\lambda} {\mathalpha}{EulerGreek}{"15}
%\DeclareMathSymbol{\mu}     {\mathalpha}{EulerGreek}{"16}
%\DeclareMathSymbol{\nu}     {\mathalpha}{EulerGreek}{"17}
%\DeclareMathSymbol{\xi}     {\mathalpha}{EulerGreek}{"18}
%\DeclareMathSymbol{\pi}     {\mathalpha}{EulerGreek}{"19}
%\DeclareMathSymbol{\rho}    {\mathalpha}{EulerGreek}{"1A}
%\DeclareMathSymbol{\sigma}  {\mathalpha}{EulerGreek}{"1B}
%\DeclareMathSymbol{\tau}    {\mathalpha}{EulerGreek}{"1C}
%\DeclareMathSymbol{\upsilon}{\mathalpha}{EulerGreek}{"1D}
%\DeclareMathSymbol{\phi}    {\mathalpha}{EulerGreek}{"1E}
%\DeclareMathSymbol{\chi}    {\mathalpha}{EulerGreek}{"1F}
%\DeclareMathSymbol{\psi}    {\mathalpha}{EulerGreek}{"20}
%\DeclareMathSymbol{\omega}  {\mathalpha}{EulerGreek}{"21}
%\DeclareMathSymbol{\varepsilon}{\mathalpha}{EulerGreek}{"22}
%\DeclareMathSymbol{\vartheta}{\mathalpha}{EulerGreek}{"23}
%\DeclareMathSymbol{\varpi}  {\mathalpha}{EulerGreek}{"24}
%\DeclareMathSymbol{\varphi} {\mathalpha}{EulerGreek}{"27}
%\DeclareMathSymbol\upOmega  {\mathord}{EulerGreek}{"0A}
%\DeclareMathSymbol\upDelta  {\mathord}{EulerGreek}{"01}

% blackbord bold letters
%\DeclareMathAlphabet{\mathds}{U}{dsrom}{m}{n}
%\usepackage[bb=fourier]{mathalfa}


==> style/ieee_additions.tex <==
% #####################
% ADDITIONS FOR LIPICS
% #####################
% some paper specific stuff

\usepackage{paralist}
\theoremstyle{plain}

\newtheorem {theorem}       {Theorem}     []
\newtheorem {corollary}		[theorem]     {Corollary}
\newtheorem {lemma}			[theorem]     {Lemma}
\newtheorem {proposition}	[theorem]     {Proposition}
\newtheorem {remark}		[theorem]     {Remark}
\newtheorem {definition}	[theorem]     {Definition}
\newtheorem {notation}		[theorem]     {Notation}
\newtheorem {example}		[theorem]     {Example}
\newtheorem {exercise}		[theorem]     {Exercise}
\newtheorem {algo}			[theorem]     {Algorithm}
\newtheorem {claim}			[theorem]     {Claim}

\sloppy
\clubpenalty = 10000 
\widowpenalty = 10000 
\displaywidowpenalty = 10000

%compact llncs-like paragraph
\newcommand{\compactparagraph}[1]{%
    \medskip%
    \noindent%
    {\bf \sffamily #1.}%
}

\newcommand{\subparagraph}[1]{%
    \medskip%
    \noindent%
    {\bf \sffamily #1.}%
}


==> style/includes.tex <==
% ##########
% INCLUDES
% ##########

% images, ...
\usepackage{graphicx}

% tables (over several pages)
%\usepackage{array}
\usepackage{tabu}
%\usepackage{longtable}

% boxes in the text
\usepackage{fancybox}

% mathematic symbols
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{stmaryrd} 
\usepackage{amsthm}
\usepackage{wasysym}

% binary ops, for comparasion only
%\usepackage{shuffle} % not compatible with LIPIcs

% colored text
\usepackage{color}

% bmatrix* with alignment
\usepackage{mathtools}

% symbol scaling in math mode
\usepackage{scalerel}

% for symbol stacking
\usepackage{stackengine}

% for coloring stuff
\usepackage{xcolor}

% \include* without new page
%\usepackage{newclude}

% parse optional arguments
\usepackage{xparse}

% subimport
\usepackage{import}

% fix some spacing issues
\usepackage{microtype}

% floating figures
\usepackage{wrapfig}

% ????
\usepackage{bm}
\usepackage{oldgerm}
\usepackage{texdraw}
\usepackage{multirow}



==> style/lang_de.tex <==
% ###################################
% LANGUAGE DEPENDANT STUFF: DEUTSCH
% ###################################

%
% Packages
%

\usepackage[ngerman]{babel}
\usepackage[utf8]{inputenc}
\usepackage{csquotes}

%
% Commands
%

\newcommand{\pts}{Punkte}
\newcommand{\page}{Seite}

\newcommand {\quot} [1] {\glqq #1\grqq}


==> style/lang_en.tex <==
% ###################################
% LANGUAGE DEPENDANT STUFF: ENGLISH
% ###################################

%
% Packages
%

%\usepackage[T1]{fontenc} % WTF!?
\usepackage[english]{babel}
\usepackage{csquotes}

%
% Commands
%

\newcommand{\pts}{points}
\newcommand{\page}{Page}

\newcommand {\quot} [1] {\enquote{#1}}


==> style/letter.tex <==
% ########################
% ARTICLE SPECIFIC STUFF
% ########################

% Festlegung Art der Zitierung - Havardmethode: Abkuerzung Autor + Jahr
\usepackage[style=alphabetic,backend=bibtex]{biblatex}

% underlining
\usepackage{ulem}

% remove all paragraph indentation
\usepackage{parskip}

% spacing between lines of text
\usepackage{setspace}

% enumerate etc
\usepackage{paralist}

% keyword index
\usepackage{makeidx}

% create keyword index
\makeindex

% abbreviation index
\usepackage[german]{nomencl}
\let\abbrev\nomenclature

% border size
\usepackage{geometry}
% top is later changed, just for title page
\geometry{left=2.5cm, right=2.5cm, top=2.5cm, bottom=2cm, foot= 1cm}

% Indentation
% space between lines
\onehalfspacing
\renewcommand{\hmmax}{0}
\renewcommand{\bmmax}{0}
\clubpenalty = 10000 % Disable single lines at the start of a paragraph (Schusterjungen)
\widowpenalty = 10000 % Disable single lines at the end of a paragraph (Hurenkinder)
\displaywidowpenalty = 10000
% Schaltet den zusätzlichen Zwischenraum ab, den LaTeX normalerweise nach einem Satzzeichen einfügt.
\frenchspacing

%\usepackage{scrpage2}
%\pagestyle{scrheadings}
%\cfoot{\pagemark}

%  headline / footline
\usepackage{fancyhdr} %Paket laden
\pagestyle{fancy} %eigener Seitenstil

%% Seitennummer immer oben rechts
%% alle Kopf- und Fußzeilenfelder bereinigen
%\fancyhf{}
%% Kopfzeile links: Name des Kapitels = der Sektion
%\fancyhead[L]{\nouppercase{\leftmark}}
%% Kopfzeile zentriert:
%\fancyhead[C]{} 
%% Kopfzeile rechts = Seitennummer
%\fancyhead[R]{\thepage} 
%% Trennlinien
%\renewcommand{\headrulewidth}{0.4pt} 
%%\renewcommand{\footrulewidth}{0.4pt}
%% Analog
%%\fancyfoot[C]{\thepage}


% Seitennummer immer oben rechts
% alle Kopf- und Fußzeilenfelder bereinigen
\fancyhf{}
\fancyfoot[C]{\thepage}
\renewcommand{\headrule}{} 

% references
\usepackage[bookmarksnumbered]{hyperref} 

% line break in URLs
%\usepackage[hyphens,obeyspaces,spaces]{url}

% newline after paragraph, paragraph bold and underlined
\makeatletter
\renewcommand {\paragraph}
{
    \@startsection
        {paragraph} % name
        {4}         % level
        {\z@}       % indent     
        {0ex \@plus -1ex \@minus -.2ex} % beforeskip
        %{-3.25ex\@plus -1ex \@minus -.2ex} % beforeskip
        {0.01ex \@plus .2ex}                % afterskip
        %{1.5ex \@plus -2ex}                % afterskip
        {\normalfont\normalsize\bfseries\underbar} % style of heading
}
\makeatother

% proof in bold font, colon and newline afterwards
\makeatletter
\renewenvironment{proof}[1][\proofname]
{
    \par
    \pushQED{\qed}%
    \normalfont \topsep6\p@\@plus6\p@\relax
    \trivlist
    \item[\hskip\labelsep\bfseries
    #1:]\mbox{}\\*\ignorespaces% ADDED
}
{
    \popQED\endtrivlist\@endpefalse
}
\makeatother

% set emph back to normal (instead of underlined)
\normalem 

% emph as bold
\makeatletter
\DeclareRobustCommand{\em}{%
    \@nomath\em \if b\expandafter\@car\f@series\@nil
    \normalfont \else \bfseries \fi}
\makeatother

% Theorem numbering
\def\theoremnumberstyle{changesection}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Zu verwendende Regelsaetze 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Bei Nummerierung vom Typ swapped soll abweichend vom Standard
%%% "5.12. Satz" erscheinen als "5.12 Satz", das heisst ohne
%%% zusaetzlichen Punkt.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\def\swappedhead#1#2#3{%
%    \thmnumber{#2}\thmname{\@ifnotempty{#2}{ }#1}%
%    \thmnote{ {\the\thm@notefont(#3)}}}

\def\swappedhead#1#2#3{%
    \thmnumber{#2}\thmname{ #1}%
    \thmnote{ {\the\thm@notefont(#3)}}}

\newtheoremstyle{varthm-roman-break}% name
{}%      Space above, empty = `usual value'
{}%      Space below
{\normalfont}% Body font
{}%         Indent amount (empty = no indent, \parindent = para indent)
{\bfseries}% Thm head font
{}%        Punctuation after thm head
{\newline}%     Space after thm head: " " = normal interword space;
%       \newline = linebreak
{\thmnote{#3}}% Thm head spec


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Eigene Befehle
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Label an beliebiger Stelle mit beliebigem Symbol setzen
% \mylabel{labelname}{(*)} liefert (*) nach \ref{labelname}
\catcode`@=11%%% Sorgt daruer, dass @ in Marconamen verwendet werden kann
\newcommand{\mylabel}[2]{\@bsphack
    \protected@write\@auxout{}%
    {\string\newlabel{#1}{{#2}{\thepage}}}%
    \@esphack}
\newcommand{\tmylabel}[2]{\@bsphack
    \protected@write\@auxout{}%
    {\string\newlabel{#1}{{#2}{\thepage}{\arabic{chapter}}}}%
    \@esphack}
\catcode`@=\active%
%%% Erzeugt an der Stelle des Aufrufs einen nicht sichtbaren Punkt.
\newcommand{\leererpunkt}{
    \drawdim pt
    \begin{texdraw}
        \setgray 1
        \lcir r:0.01       
    \end{texdraw}
}

\swapnumbers
\theoremstyle{varthm-roman-break} 

\newtheorem {theorem}	    {Theorem}     [section]
\newtheorem {corollary}		[theorem]     {Corollary}
\newtheorem {lemma}			[theorem]     {Lemma}
\newtheorem {proposition}	[theorem]     {Proposition}
\newtheorem {remark}		[theorem]     {Remark}
\newtheorem {definition}	[theorem]     {Definition}
\newtheorem {notation}		[theorem]     {Notation}
\newtheorem {example}		[theorem]     {Example}
\newtheorem {exercise}		[theorem]     {Example}
\newtheorem {algo}			[theorem]     {Algorithm}
\newtheorem {claim}			[theorem]     {Claim}

% itemize/enumerate at the beginning of a thm
\newenvironment{thmenumerate}
{
    \leavevmode\vspace{-1.4em}
    \begin{enumerate}
    }
    {
    \end{enumerate}
}

\newenvironment{thmitemize}
{
    \leavevmode\vspace{-1.4em}
    \begin{itemize}
    }
    {
    \end{itemize}
}

% chapters = sections (otherwise numbering will not work)
\let\chapter\section

% subsections numbered by capital arabic letters
%\renewcommand{\thesubsection}{\thesection.\Roman{subsection}}
\renewcommand{\thesubsection}{\Alph{subsection})}

\usepackage{secdot}
\sectionpunct{subsection}{ }


% captions
\usepackage{capt-of}
\usepackage{caption}
\DeclareCaptionFont{white}{\color{white}}
\DeclareCaptionFormat{listing}
{
    \colorbox[cmyk]{1, 1, 1,0.01}
    {
        \parbox{\textwidth}
        {\hspace{15pt}#1#2#3}
    }
}
\captionsetup[lstlisting]
{
    format=listing,
    labelfont=white,
    textfont=white,
    singlelinecheck=false,
    margin=0pt,
    font={bf,footnotesize}
}

% listings
\usepackage{listings}
\lstset{
    numbers=left,
    numberstyle=\tiny,
    numbersep=5pt,
    keywordstyle=\color{black}\bfseries,
    stringstyle=\ttfamily,
    showstringspaces=false,
    basicstyle=\footnotesize,
    captionpos=b
}
\lstset{language=java}
% Listings
\lstset{
    basicstyle=\fontsize{9}{9}\ttfamily, % Standardschrift
    numbers=left,               % Ort der Zeilennummern
    numberstyle=\tiny,          % Stil der Zeilennummern
    %stepnumber=2,               % Abstand zwischen den Zeilennummern
    numbersep=5pt,              % Abstand der Nummern zum Text
    tabsize=4,                  % Groesse von Tabs
    extendedchars=true,         %
    breaklines=true,            % Zeilen werden Umgebrochen
    keywordstyle=\text,
    %frame=b,         
    stringstyle=\color{black}\ttfamily, % Farbe der String
    showspaces=false,           % Leerzeichen anzeigen ?
    showtabs=false,             % Tabs anzeigen ?
    xleftmargin=5pt,
    framexleftmargin=17pt,
    framexrightmargin=5pt,
    framexbottommargin=4pt,
    %backgroundcolor=\color{lightgray},
    showstringspaces=false,      % Leerzeichen in Strings anzeigen ?
    captionpos=t,     
}

\lstloadlanguages{% Check Dokumentation for further languages ...
    %[Visual]Basic
    %Pascal
    %C
    %C++
    %XML
    %HTML
    Java
}

\definecolor{myblue}{HTML}{3399FF}
\definecolor{mybluefaded}{HTML}{99CCFF}
\definecolor{myred}{HTML}{FF3333}
\definecolor{myredfaded}{HTML}{FF9999}


\newtoks\receiver
\newtoks\address
\newtoks\postalbox
\newtoks\plz
\newtoks\telnr
\newtoks\email

\catcode`\@ = 11 % Macro \makeatletter does the same

%\newcommand{ \at } { \makeatletter @ \makeatother }

\newcommand {\letterhead}
{
    
    \begin{tabularx}{\textwidth}{lXr}
        \large \the\receiver       & & \large Sebastian Muskalla\\
        \small \the\address     & & \small TU Kaiserslautern, Concurrency Theory Group\\
        \small \the\postalbox  & & \small Postfach 3049\\
        \small \the\plz       & & \small 67663 Kaiserslautern\\
        \small \the\telnr     & & \small Tel.:  +49 (0)631 205 3051 \\
        \small \the\email     & & \small E-Mail: muskalla{\!\at \!}cs.uni-kl.de\\
                                & & \\
                                & & Kaiserslautern, den \today \\
    \end{tabularx}
    \makeatother
}

\newcommand {\lettertitle}
{\mbox{}\\\textbf{\Large{\@title}}\\}




==> style/lipics_additions.tex <==
% #####################
% ADDITIONS FOR LIPICS
% #####################
% some paper specific stuff

\usepackage{paralist}
\theoremstyle{plain}
\newtheorem {proposition} [theorem] {Proposition}
\newtheorem {Claim} [theorem] {Claim}

\theoremstyle{definition}
\newtheorem {algo} [theorem] {Algorithm}

\sloppy
\clubpenalty = 10000 
\widowpenalty = 10000 
\displaywidowpenalty = 10000

%compact llncs-like paragraph
\newcommand{\compactparagraph}[1]{%
    \medskip%
    \noindent%
    {\bf \sffamily #1.}%
}


==> style/misc.tex <==
% ##########
% MISC
% ##########

% FIX DELIMITERS SPACING
\let\originalleft\left
\let\originalright\right
\renewcommand{\left}{\mathopen{}\mathclose\bgroup\originalleft}
\renewcommand{\right}{\aftergroup\egroup\originalright}

% triangle qed
\newcommand{\tqed}{\hfill \text{$\blacktriangleleft$}}

% item with arrow symbol like in Meyer's lectures
\newcommand {\itemarrow} 
{ {\raisebox{0.8mm}{\rotatebox[origin=c]{180}{$\Lsh$}}} }

% skip line (for nice enumerate / itemize)
\newcommand {\skipline}
{
    \mbox{}
    \vspace*{-0.3cm}
}

% brackets in various sizes
%\newcommand {\ob} {\big (}
%\newcommand {\obm} {\Big (}
%\newcommand {\obl} {\bigg (}
%\newcommand {\obh} {\Bigg (}
%\newcommand {\cb} {\big )}
%\newcommand {\cbm} {\Big )}
%\newcommand {\cbl} {\bigg )}
%\newcommand {\cbh} {\Bigg )}
%
%\newcommand {\osb} {\big [}
%\newcommand {\osbm} {\Big [}
%\newcommand {\osbl} {\bigg [}
%\newcommand {\osbh} {\Bigg [}
%\newcommand {\csb} {\big [}
%\newcommand {\csbm} {\Big ]}
%\newcommand {\csbl} {\bigg ]}
%\newcommand {\csbh} {\Bigg ]}



==> style/myriad.tex <==
% #######
% MYRIAD
% #######

% REQUIRES XELATEX!

% Consolas and Myriad Pro have to be installed

% - upright myriad for text
% - italic myriad formath
% - consolas for monospace
% - euler for greek letters

% package to change font in XeTeX
\usepackage[no-math]{fontspec}

% euler font for math
\usepackage[mathbf]{euler}
    
% default font: Myriad pro
% (has to be installed!)
\setmainfont{Myriad Pro}
\newfontfamily\myriad{Myriad Pro}

% monospace font: Consolas
% (has to be installed!)
\setmonofont{Consolas}

% use normal text font for math
\usepackage[noendash,italic]{mathastext}

% hack for emptyset
\renewcommand{\emptyset}{ {\diameter} }

% font for section, part, ... titles (in text and in table of contents)
\addtokomafont{title}{\myriad}
\setkomafont{subsection}{\bfseries\Large\myriad}
\setkomafont{section}{\bfseries\huge\myriad}
\setkomafont{sectionentry}{\bfseries\myriad} % entry in TOC
\setkomafont{part}{\bfseries\Huge\myriad} % part name
\setkomafont{partnumber}{\bfseries\Huge\myriad} % "Part II."
\setkomafont{partentry}{\bfseries\large\myriad} % entry in TOC
\setkomafont{paragraph}{\bfseries\myriad}
\setkomafont{subparagraph}{\bfseries\myriad} % entry in TOC

% Take nice sans-serif greek letters from the font "Euler"
%\DeclareSymbolFont{EulerGreek}{U}{eur}{m}{n}
%\DeclareMathSymbol\Gamma    {\mathalpha}{EulerGreek}{"00}
%\DeclareMathSymbol\Delta    {\mathalpha}{EulerGreek}{"01}
%\DeclareMathSymbol\Theta    {\mathalpha}{EulerGreek}{"02}
%\DeclareMathSymbol\Lambda   {\mathalpha}{EulerGreek}{"03}
%\DeclareMathSymbol\Xi       {\mathalpha}{EulerGreek}{"04}
%\DeclareMathSymbol\Pi       {\mathalpha}{EulerGreek}{"05}
%\DeclareMathSymbol\Sigma    {\mathalpha}{EulerGreek}{"06}
%\DeclareMathSymbol\Upsilon  {\mathalpha}{EulerGreek}{"07}
%\DeclareMathSymbol\Phi      {\mathalpha}{EulerGreek}{"08}
%\DeclareMathSymbol\Psi      {\mathalpha}{EulerGreek}{"09}
%\DeclareMathSymbol\Omega    {\mathalpha}{EulerGreek}{"0A}
%\DeclareMathSymbol{\alpha}  {\mathalpha}{EulerGreek}{"0B}
%\DeclareMathSymbol{\beta}   {\mathalpha}{EulerGreek}{"0C}
%\DeclareMathSymbol{\gamma}  {\mathalpha}{EulerGreek}{"0D}
%\DeclareMathSymbol{\delta}  {\mathalpha}{EulerGreek}{"0E}
%\DeclareMathSymbol{\epsilon}{\mathalpha}{EulerGreek}{"0F}
%\DeclareMathSymbol{\zeta}   {\mathalpha}{EulerGreek}{"10}
%\DeclareMathSymbol{\eta}    {\mathalpha}{EulerGreek}{"11}
%\DeclareMathSymbol{\theta}  {\mathalpha}{EulerGreek}{"12}
%\DeclareMathSymbol{\iota}   {\mathalpha}{EulerGreek}{"13}
%\DeclareMathSymbol{\kappa}  {\mathalpha}{EulerGreek}{"14}
%\DeclareMathSymbol{\lambda} {\mathalpha}{EulerGreek}{"15}
%\DeclareMathSymbol{\mu}     {\mathalpha}{EulerGreek}{"16}
%\DeclareMathSymbol{\nu}     {\mathalpha}{EulerGreek}{"17}
%\DeclareMathSymbol{\xi}     {\mathalpha}{EulerGreek}{"18}
%\DeclareMathSymbol{\pi}     {\mathalpha}{EulerGreek}{"19}
%\DeclareMathSymbol{\rho}    {\mathalpha}{EulerGreek}{"1A}
%\DeclareMathSymbol{\sigma}  {\mathalpha}{EulerGreek}{"1B}
%\DeclareMathSymbol{\tau}    {\mathalpha}{EulerGreek}{"1C}
%\DeclareMathSymbol{\upsilon}{\mathalpha}{EulerGreek}{"1D}
%\DeclareMathSymbol{\phi}    {\mathalpha}{EulerGreek}{"1E}
%\DeclareMathSymbol{\chi}    {\mathalpha}{EulerGreek}{"1F}
%\DeclareMathSymbol{\psi}    {\mathalpha}{EulerGreek}{"20}
%\DeclareMathSymbol{\omega}  {\mathalpha}{EulerGreek}{"21}
%\DeclareMathSymbol{\varepsilon}{\mathalpha}{EulerGreek}{"22}
%\DeclareMathSymbol{\vartheta}{\mathalpha}{EulerGreek}{"23}
%\DeclareMathSymbol{\varpi}  {\mathalpha}{EulerGreek}{"24}
%\DeclareMathSymbol{\varphi} {\mathalpha}{EulerGreek}{"27}
%\DeclareMathSymbol\upOmega  {\mathord}{EulerGreek}{"0A}
%\DeclareMathSymbol\upDelta  {\mathord}{EulerGreek}{"01}

% blackbord bold letters
%\DeclareMathAlphabet{\mathds}{U}{dsrom}{m}{n}
\usepackage[bb=fourier]{mathalfa}


==> style/nth.tex <==
% nth.sty  version 2002/27/02 Donald Arseneau
% Ordinal numbering style, 1st 2nd 3rd 4th 5th... 12th... 101st 102nd...
%
% (Public domain: take, include, extract, whatever)
%
% In LaTeX: 
%           \usepackage[super,negative]{nth}
% where option [super] gives superscript `th'
% and option [negative] allows ``st, nd, rd'' suffixes on negative numbers.
%
% example:  \renewcommand{\thesection}{\ordinal{section}}
% or        \renewcommand{\thesection}{\@ordinal\c@section}
% or        \renewcommand{\thesection}{\nth\c@section}
%   
% In plain TeX: 
%           \input nth.sty
% use:      \nth{<number>}.
% Change formatting by redefining \nthscript and \nthtest

% modified to be also able to do things like \nth{i}
% (in this case, always "th" is used)

% ToDo:
% \nth{(n+1)} should give (n+1)^st

\usepackage{xstring}

\def\nth#1{
    \IfInteger{#1}
    {\nthH{#1}}
    {#1\nthscript{th}}
}

\def\nthH#1{% First print number:
    \expandafter\nthM \number #1\relax
    \nthscript{%
        \ifnum#1\nthtest0 th\else % negatives are all ``th'' (depending on \nthtest)
        \expandafter \nthSuff \expandafter 0\number\ifnum #1<0-\fi#1\delimiter
        \fi
    }}
    
% Minus sign using math mode:
\def\nthM#1{\if -#1\ifmmode-\else$-$\fi\else #1\fi}

% Print suffix depending on last two digits:
\def\nthSuff#1#2#3{%
    \ifx \delimiter#3% #1#2 are last two digits
    \ifnum #1=1 th%  teens are always ``th''
    \else % use appropriate suffix
    \ifcase #2 th\or st\or nd\or rd\else th\fi
    \fi
    \else % continue scanning for last two digits
    \expandafter \nthSuff \expandafter #2\expandafter #3%
    \fi}

% Formatting hook for ordinals (\let\nthscript\textsuperscript)
\def\nthscript#1{\textsuperscript{#1}}% alternate: \def\nthscript#1{$\rm^{#1}$}

% Formatting hook for all negative numbers giving ``th''
\def\nthtest{=}  % alternate: \def\nthtest{=}

%\ifx\Alph\undefined\else
%\def\ordinal#1{\expandafter\@ordinal\csname c@#1\endcsname}
%\let\@ordinal\nth
%\ProvidesPackage{smnth}[2016/05/31] % yyyy-mm-dd
%\DeclareOption{super}{\def\nthscript#1{#1}}
%\DeclareOption{negative}{\def\nthtest{<}}
%\ProcessOptions
%\fi
%    


==> style/operators.tex <==
% ##################
% OPERATORS
% ##################

\DeclareMathOperator {\characteristic} {char}
\DeclareMathOperator {\cols} {cols}
\DeclareMathOperator {\rows} {rows}
\DeclareMathOperator{\Attr}{Attr}
\DeclareMathOperator{\ann}{ann}
\DeclareMathOperator{\Ass}{Ass}
\DeclareMathOperator{\Aut}{Aut}
\DeclareMathOperator{\Baselocus}{Baselocus}
\DeclareMathOperator{\Bil}{Bil}
\DeclareMathOperator{\Bl}{Bl}
\DeclareMathOperator{\Char}{char}
\DeclareMathOperator{\Cl}{\kc\!\!\;\ell\!\:}
\DeclareMathOperator{\codim}{codim}
\DeclareMathOperator{\Cok}{Cok}
\DeclareMathOperator{\coker}{coker}
\DeclareMathOperator{\degbound}{d}
\DeclareMathOperator{\Def}{Def}
\DeclareMathOperator{\Der}{Der}
\DeclareMathOperator{\Div}{Div}
\DeclareMathOperator{\Eig}{Eig}
\DeclareMathOperator{\End}{End}
\DeclareMathOperator{\Exp}{Exp}
\DeclareMathOperator{\expdim}{expdim}
\DeclareMathOperator{\Ext}{Ext}
\DeclareMathOperator{\Fix}{Fix}
\DeclareMathOperator{\Gal}{Gal}
\DeclareMathOperator{\GF}{GF}
\DeclareMathOperator{\ggT}{ggT}
\DeclareMathOperator{\ggt}{ggt}
\DeclareMathOperator{\Gl}{Gl}
\DeclareMathOperator{\Gr}{Gr}
\DeclareMathOperator{\Graph}{Graph}
\DeclareMathOperator{\height}{height}
\DeclareMathOperator{\Hau}{Hau}
\DeclareMathOperator{\Hom}{Hom}
\DeclareMathOperator{\Hilb}{Hilb}
\DeclareMathOperator{\HP}{HP}
%{\HOM}[1]{\mbox{\DeclareFixedFont{\AZC}{T1}{pzc}{m}{it}{#1}\AZC Hom\,}}
\DeclareMathOperator{\Ker}{Ker}
\DeclareMathOperator{\kgV}{kgV}
\DeclareMathOperator{\kgv}{kgv}
\DeclareMathOperator{\lc}{lc}
\DeclareMathOperator{\lead}{lead}
\DeclareMathOperator{\length}{length}
\DeclareMathOperator{\id}{id}
\DeclareMathOperator{\im}{Im}
\DeclareMathOperator{\ind}{ind}
\DeclareMathOperator{\Inn}{Inn}
\DeclareMathOperator{\inv}{inv}
\DeclareMathOperator{\jet}{jet}
\DeclareMathOperator{\lcm}{lcm}
\DeclareMathOperator{\Lin}{Lin}
\DeclareMathOperator{\Mat}{Mat}
%\renewcommand{\mod}{\mbox{\rm mod }}
\DeclareMathOperator{\modality}{mod}
\DeclareMathOperator{\Mon}{Mon}
\DeclareMathOperator{\Mor}{Mor}
%\DeclareMathOperator{\mSpec}{\textswab{m}-Spec}
\DeclareMathOperator{\mult}{mult}
\DeclareMathOperator{\NS}{NS}
\DeclareMathOperator{\Num}{Num}
\DeclareMathOperator{\ord}{ord}
\DeclareMathOperator{\OO}{O}
\DeclareMathOperator{\Pic}{Pic}
\DeclareMathOperator{\Pot}{Pot}
\DeclareMathOperator{\pr}{pr}
\DeclareMathOperator{\Preshv}{Preshv}
\DeclareMathOperator{\Proj}{Proj}
\DeclareMathOperator{\PGL}{PGL}
\DeclareMathOperator{\PSL}{PSL}
\DeclareMathOperator{\Quot}{Quot}
\DeclareMathOperator{\rang}{rang}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\re}{Re}
%\DeclareMathOperator{\Res}{Res}
\DeclareMathOperator{\Reg}{Reg}
\DeclareMathOperator{\Sec}{Sec}
\DeclareMathOperator{\Sesq}{Sesq}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Sing}{Sing}
\DeclareMathOperator{\Shv}{Shv}
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\Sl}{Sl}
\DeclareMathOperator{\SO}{SO}
\DeclareMathOperator{\Spec}{Spec}
\DeclareMathOperator{\Spur}{Spur}
\DeclareMathOperator{\SU}{SU}
\DeclareMathOperator{\Syl}{Syl}
\DeclareMathOperator{\val}{val}
\DeclareMathOperator{\Sym}{Sym}
\DeclareMathOperator{\Tor}{Tor}
\DeclareMathOperator{\UU}{U}
\DeclareMathOperator{\ZFK}{ZFK}
\DeclareMathOperator{\redNF}{redNF}
\DeclareMathOperator{\spoly}{spoly}
\DeclareMathOperator{\tail}{tail}
\DeclareMathOperator{\new}{new}
\DeclareMathOperator{\bin}{bin}
%\DeclareMathOperator{\st}{s.t.}


==> style/presentation.tex <==
% #######################
% BEAMER SPECIFIC STUFF
% #######################

% Metropolis theme
% (has to be installed)
\usetheme{metropolis}

% ???
\usepackage{booktabs}
\usepackage[scale=2]{ccicons}

% stuff for tikz
\usepackage{pgfplots}
\usepgfplotslibrary{dateplot}

% absolute positioning of boxes
\usepackage[absolute,overlay]{textpos}

% enumeration
\usepackage{enumerate}

% emph as bold
\makeatletter
\DeclareRobustCommand{\em}{%
    \@nomath\em \if b\expandafter\@car\f@series\@nil
    \normalfont \else \bfseries \fi}
\makeatother

\definecolor{myblue}{HTML}{3399FF}
\definecolor{mybluefaded}{HTML}{99CCFF}
\definecolor{myred}{HTML}{FF3333}
\definecolor{myredfaded}{HTML}{FF9999}



==> style/stix.tex <==
% #######
% MYRIAD
% #######


% - myriad for text and math
% - consolas for monospace
% - euler for greek letters

% REQUIRES XELATEX!

% Consolas and Myriad Pro have to be installed

% Myriad pro for text (and math)
% Consolas for monospace
% Euler for math

\usepackage[notext]{stix}

% package to change font in XeTeX
\usepackage[no-math]{fontspec}

% euler font for math
%\usepackage[mathbf]{euler}
    
% default font: Myriad pro
% (has to be installed!)
\setmainfont{Myriad Pro}
\newfontfamily\myriad{Myriad Pro}

% monospace font: Consolas
% (has to be installed!)
\setmonofont{Consolas}

% use normal text font for math
%\usepackage[noendash,italic]{mathastext}

% hack for emptyset
\renewcommand{\emptyset}{ {\diameter} }

% font for section, part, ... titles (in text and in table of contents)
\usepackage{titlesec}
\addtokomafont{title}{\myriad}
\setkomafont{subsection}{\bfseries\Large\myriad}
\setkomafont{section}{\bfseries\huge\myriad}
\setkomafont{sectionentry}{\bfseries\myriad} % entry in TOC
\setkomafont{part}{\bfseries\Huge\myriad} % part name
\setkomafont{partnumber}{\bfseries\Huge\myriad} % "Part II."
\setkomafont{partentry}{\bfseries\large\myriad} % entry in TOC
\setkomafont{paragraph}{\bfseries\myriad}
\setkomafont{subparagraph}{\bfseries\myriad} % entry in TOC

% Take nice sans-serif greek letters from the font "Euler"
%\DeclareSymbolFont{EulerGreek}{U}{eur}{m}{n}
%\DeclareMathSymbol\Gamma    {\mathalpha}{EulerGreek}{"00}
%\DeclareMathSymbol\Delta    {\mathalpha}{EulerGreek}{"01}
%\DeclareMathSymbol\Theta    {\mathalpha}{EulerGreek}{"02}
%\DeclareMathSymbol\Lambda   {\mathalpha}{EulerGreek}{"03}
%\DeclareMathSymbol\Xi       {\mathalpha}{EulerGreek}{"04}
%\DeclareMathSymbol\Pi       {\mathalpha}{EulerGreek}{"05}
%\DeclareMathSymbol\Sigma    {\mathalpha}{EulerGreek}{"06}
%\DeclareMathSymbol\Upsilon  {\mathalpha}{EulerGreek}{"07}
%\DeclareMathSymbol\Phi      {\mathalpha}{EulerGreek}{"08}
%\DeclareMathSymbol\Psi      {\mathalpha}{EulerGreek}{"09}
%\DeclareMathSymbol\Omega    {\mathalpha}{EulerGreek}{"0A}
%\DeclareMathSymbol{\alpha}  {\mathalpha}{EulerGreek}{"0B}
%\DeclareMathSymbol{\beta}   {\mathalpha}{EulerGreek}{"0C}
%\DeclareMathSymbol{\gamma}  {\mathalpha}{EulerGreek}{"0D}
%\DeclareMathSymbol{\delta}  {\mathalpha}{EulerGreek}{"0E}
%\DeclareMathSymbol{\epsilon}{\mathalpha}{EulerGreek}{"0F}
%\DeclareMathSymbol{\zeta}   {\mathalpha}{EulerGreek}{"10}
%\DeclareMathSymbol{\eta}    {\mathalpha}{EulerGreek}{"11}
%\DeclareMathSymbol{\theta}  {\mathalpha}{EulerGreek}{"12}
%\DeclareMathSymbol{\iota}   {\mathalpha}{EulerGreek}{"13}
%\DeclareMathSymbol{\kappa}  {\mathalpha}{EulerGreek}{"14}
%\DeclareMathSymbol{\lambda} {\mathalpha}{EulerGreek}{"15}
%\DeclareMathSymbol{\mu}     {\mathalpha}{EulerGreek}{"16}
%\DeclareMathSymbol{\nu}     {\mathalpha}{EulerGreek}{"17}
%\DeclareMathSymbol{\xi}     {\mathalpha}{EulerGreek}{"18}
%\DeclareMathSymbol{\pi}     {\mathalpha}{EulerGreek}{"19}
%\DeclareMathSymbol{\rho}    {\mathalpha}{EulerGreek}{"1A}
%\DeclareMathSymbol{\sigma}  {\mathalpha}{EulerGreek}{"1B}
%\DeclareMathSymbol{\tau}    {\mathalpha}{EulerGreek}{"1C}
%\DeclareMathSymbol{\upsilon}{\mathalpha}{EulerGreek}{"1D}
%\DeclareMathSymbol{\phi}    {\mathalpha}{EulerGreek}{"1E}
%\DeclareMathSymbol{\chi}    {\mathalpha}{EulerGreek}{"1F}
%\DeclareMathSymbol{\psi}    {\mathalpha}{EulerGreek}{"20}
%\DeclareMathSymbol{\omega}  {\mathalpha}{EulerGreek}{"21}
%\DeclareMathSymbol{\varepsilon}{\mathalpha}{EulerGreek}{"22}
%\DeclareMathSymbol{\vartheta}{\mathalpha}{EulerGreek}{"23}
%\DeclareMathSymbol{\varpi}  {\mathalpha}{EulerGreek}{"24}
%\DeclareMathSymbol{\varphi} {\mathalpha}{EulerGreek}{"27}
%\DeclareMathSymbol\upOmega  {\mathord}{EulerGreek}{"0A}
%\DeclareMathSymbol\upDelta  {\mathord}{EulerGreek}{"01}

% blackbord bold letters
%\DeclareMathAlphabet{\mathds}{U}{dsrom}{m}{n}
\usepackage[bb=fourier]{mathalfa}


==> style/theorems_de.tex <==
% ######################
% THEOREM ENVIRONMENTS
% ######################


\newtheorem {corollary}		[theorem]     {Korollar}
\newtheorem {lemma}			[theorem]     {Lemma}
\newtheorem {proposition}	[theorem]     {Proposition}
\newtheorem {remark}		[theorem]     {Bemerkung}
\newtheorem {definition}	[theorem]     {Definition}
\newtheorem {notation}		[theorem]     {Notation}
\newtheorem {example}		[theorem]     {Beispiel}
\newtheorem {exercise}		[theorem]     {Aufgabe}
\newtheorem {algo}			[theorem]     {Algorithmus}
\newtheorem {claim}			[theorem]     {Behauptung}


==> style/theorems_en.tex <==
% ######################
% THEOREM ENVIRONMENTS
% ######################

%\newtheorem {theorem}	    {Theorem}     [section]
\newtheorem {corollary}		[theorem]     {Corollary}
\newtheorem {lemma}			[theorem]     {Lemma}
\newtheorem {proposition}	[theorem]     {Proposition}
\newtheorem {remark}		[theorem]     {Remark}
\newtheorem {definition}	[theorem]     {Definition}
\newtheorem {notation}		[theorem]     {Notation}
\newtheorem {example}		[theorem]     {Example}
\newtheorem {exercise}		[theorem]     {Exercise}
\newtheorem {algo}			[theorem]     {Algorithm}
\newtheorem {claim}			[theorem]     {Claim}


==> style/tikz.tex <==
% ########################
% TIKZ
% ########################

% Includes
\usepackage{tikz}
\usepackage{pgf}

\usetikzlibrary{external}
\tikzexternalize[prefix=tikz_external/]

\usetikzlibrary{arrows}
\usetikzlibrary{automata}
\usetikzlibrary{shapes}
\usetikzlibrary{backgrounds}
\usetikzlibrary{petri}
\usetikzlibrary{calc} 
\usetikzlibrary{decorations}
\usetikzlibrary{decorations.markings}
\usetikzlibrary{decorations.pathmorphing}

\tikzset{
    treenode/.style = {align=center, inner sep=0pt, text centered,
        font=\sffamily},
    arn_n/.style = {treenode, circle, white, font=\sffamily\bfseries, draw=black,
        fill=black, text width=1.5em},% arbre rouge noir, noeud noir
    arn_r/.style = {treenode, circle, red, draw=red, 
        text width=1.5em, very thick},% arbre rouge noir, noeud rouge
    arn_x/.style = {treenode, rectangle, draw=black,
        minimum width=0.5em, minimum height=0.5em},% arbre rouge noir, nil
    roundpos/.style = {treenode, circle, black, draw=black,
        minimum size=2.5em},
    squarepos/.style = {treenode, rectangle, black, draw=black,
        minimum width=2em, minimum height=2em},
}
\tikzset{
    invisible/.style={opacity=0},
    visible on/.style={alt={#1{}{invisible}}},
    alt/.code args={<#1>#2#3}{%
        \alt<#1>{\pgfkeysalso{#2}}{\pgfkeysalso{#3}} % \pgfkeysalso doesn't change the path
    },
}

\tikzset
{
    tboxoutline/.style = 
    {
        draw,
        thick,
        minimum size=6em,
        inner sep=0pt,
        outer sep=0pt,
    },
    tboxstate/.style =
    {
        minimum width=4pt,
        minimum height=2pt,
        inner sep=0pt,
        fill
    },
    tboxarrow/.style =
    {
    },
    pics/tbox/.style 2 args =
    {
        code =
        {
            \node[tboxoutline,pic actions] (-box) {};
            \foreach \i in {1,...,#1}
            {
                \path
                    (-box.north west)
                    --
                    node
                        [tboxstate,anchor=east,pos=-1/#1/2+\i/#1,pic actions]
                        (-box-in-\i)
                        {}
                    (-box.south west);
                \path
                    (-box.north east) --
                    node
                        [tboxstate,anchor=west,pos=-1/#1/2+\i/#1,pic actions]
                        (-box-out-\i)
                        {}
                (-box.south east);
            }
            
            \foreach \i/\j/\d in {#2}
            {
                \draw
                    [   
                        tboxarrow,
                        decoration =
                        {
                            markings,
                            mark=
                                at position 1 with
                                {
                                    \arrow[scale=1,>=triangle 45]{>}
                                }
                        }
                        ,
                        postaction={decorate}
                    ]
                    (-box-in-\i.east)
                    --
                    node
                        [pos=.8,\d]
                        {}
                    (-box-out-\j.west);
            }
        }
    },
    tbox color/.style={
        tboxstate/.append style={fill=#1},
        tboxoutline/.append style={draw=#1},
        tboxarrow/.append style={draw=#1},
    },
    trans/.style =
    {
        thick,
    },
    dot/.style =
    {
        circle,
        draw,
        minimum size=6pt,
        inner sep=0pt,
        fill,
    },
}

